DREAM: A Dynamic Scheduler for Dynamic Real-time Multi-model ML Workloads

Emerging real-time multi-model ML (RTMM) workloads such as AR/VR and drone control involve dynamic behaviors in various granularity; task, model, and layers within a model. Such dynamic behaviors introduce new challenges to the system software in an ML system since the overall system load is not completely predictable, unlike traditional ML workloads. In addition, RTMM workloads require real-time processing, involve highly heterogeneous models, and target resource-constrained devices. Under such circumstances, developing an effective scheduler gains more importance to better utilize underlying hardware considering the unique characteristics of RTMM workloads. Therefore, we propose a new scheduler, DREAM, which effectively handles various dynamicity in RTMM workloads targeting multi-accelerator systems. DREAM quantifies the unique requirements for RTMM workloads and utilizes the quantified scores to drive scheduling decisions, considering the current system load and other inference jobs on different models and input frames. DREAM utilizes tunable parameters that provide fast and effective adaptivity to dynamic workload changes. In our evaluation of five scenarios of RTMM workload, DREAM reduces the overall UXCost, which is an equivalent metric of the energy-delay product (EDP) for RTMM defined in the paper, by 32.2% and 50.0% in the geometric mean (up to 80.8% and 97.6%) compared to state-of-the-art baselines, which shows the efficacy of our scheduling methodology.

==> algorithms/alg_scheduler.tex <==
\begin{algorithm}[h]
\caption{\hl{\mbox{\scheduler} scheduling algorithm}} \label{alg:scheduling_alg}
\begin{algorithmic}[1]

\LeftComment{\textbf{Input>} \textbf{ReqQues} (Request Queues), \textbf{Md} (A list of models in the workload), \textbf{AccList} (A list of accelerators), $\bm{T_{exec}}$ (A time window where we run workloads)}
\LeftComment{\textbf{Output>} }

\State{$AccStatus[len(AccList)] = \{IDLE,\}$}

\While{!ReqQue.empty}
    \For{$acc \ \text{\textbf{in}} \ AccList$}
        \If{AccStatus[acc] == COMPLETE} 
            \State $AccStatus[acc] \leftarrow IDLE$
        \EndIf

    
    \EndFor
    \For {acc\_id in range(K)}
    \LeftComment{\% If acc\_id finishes running the current layer \%}
        \If{acc\_id is done}
            \State $\mathrm{eventTime} \leftarrow \mathrm{time(acc\_id)}$
            \State $\mathrm{que\_id} \leftarrow \mathrm{queue(acc\_id)}$
            \State $To\_go_{que\_id}\ \textrm{-=}\ \mathrm{Average(Layer_{que\_id}\ latency)}$

            \State BusyArray[acc\_id] = IDLE
            \LeftComment{\% If the task finishes, dequeue \%}
            \If{ReqQue(que\_id) is done}
                \State ReqQue(que\_id).deque()
            \EndIf 
        \EndIf
    \EndFor
    \LeftComment{\% New dispatched task: get overall $To\_go$ \% }
    \LeftComment{\% Average: average latency of all accelerators \%}
    \For {que\_id in range(N)}
        \If{$\mathrm{ReqQue(que\_id)}$ newly dispatched}
            %\State $To\_go_{que\_id} = 0$
            \For{$\mathrm{Layer_{i}}$ in Layers}    
                \State $To\_go_{que\_id}\ \textrm{+=}\ \mathrm{Average(Layer_{i}\ latency)}$
            \EndFor
            \State $\mathrm{eventTime} \leftarrow \mathrm{ReqQue(que\_id).dispatch\_time}$
        \EndIf
    \EndFor

    \LeftComment{\% Get IDLE accelerator indices \%}
    \For {acc\_id in range(K)}:
        \State IdleAcc = []
        \If {BusyArray[acc\_id] == IDLE:}
		\State IdleAcc::accId
        \EndIf
    \EndFor
    %\State $\mathrm{M} \leftarrow \mathrm{len(IdleAcc)}$
    \State MapScore[len(IdleAcc)][N] = [0]
    
    %\While{!IdleAcc.empty \&\& !ReqQue.empty}
    \LeftComment{\% Iterate over ReqQue(j) and IdleAcc(i) \%}
    \For{j in range(N)}
        \For {i in range(len(IdleAcc))}
            \If{ReqQue(j) is busy}
                \State \textbf{continue}
            \EndIf
            \State $\mathrm{acc\_id} \leftarrow \mathrm{IdleAcc[i]}$
            %acc (accel type), i (task ID), curr_time (current time), prev_i (previous task ID)
            \State $\mathrm{MapScore[i][j]} \leftarrow \mathrm{Alg1(acc\_id, j, eventTime)}$
        \EndFor
    \EndFor
    \LeftComment{\% Schedule accelerator in the order of the sum of \scoreMetric of candidate tasks \%}
    \State MapScore.sorted(sum of axis=1, descending order)
    %\State S[M] = sum(MapScore, axis=1)
    %\State MapScore = [x for y, x in sorted(zip(S, MapScore), reversed)]
    \For {i in range(len(IdleAcc))}
        \If{MapScore == [0]}
            \State \textbf{break}
        \EndIf
        \LeftComment{\% Select the task with highest \scoreMetric \%}
        \State $\mathrm{idx} \leftarrow \mathrm{getIndex(MapScore[i].max)}$
        %\LeftComment{\% For selected task, update To\_go cycle \%}
        %State $To\_go_{idx}\ \textrm{-=}\ \mathrm{Average(Layer_{idx}\ latency)}$
        \State MapScore[:][idx] = [0]
    \EndFor
     
\EndWhile



\end{algorithmic}

\end{algorithm}

==> include/packages.tex <==

%\usepackage{amsmath}
%\usepackage{amsfonts}
%\usepackage{amsthm}
\theoremstyle{definition}
\newtheorem{definition}{Definition}

%\usepackage{algorithmic}
%\usepackage[linesnumbered]{algorithm2e}
\usepackage{color}
%\usepackage{cite}
\usepackage[normalem]{ulem}

% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{xspace}
\usepackage{graphicx}
\usepackage{subfigure}
%\usepackage{subcaption}
\usepackage{booktabs} % for professional tables

\usepackage{multirow}
\usepackage{comment}

% hyperref makes hyperlinks in the resulting PDF.
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
% \usepackage{mlsys2021} with \usepackage[nohyperref]{mlsys2021} above.
\usepackage{hyperref}
\usepackage{bm}



\RequirePackage[nameinlink]{cleveref} % 'nameinlink' to mimic \autoref's behavior
%% Use low-level controls to hard-code the required appearance.
\crefname{chapter}{Chapter}{Chapters}
\crefname{section}{Section}{Sections}
\crefname{subsection}{Section}{Sections}
\crefname{equation}{Equation}{Equations}
\crefname{definition}{Definition}{Definitions}
\crefname{assumption}{Assumption}{Assumptions}
\crefname{theorem}{Theorem}{Theorems}
\crefname{figure}{Figure}{Figures}
\crefname{table}{Table}{Tables}
\crefname{algorithm}{Algorithm}{Algorithms}
% etc
\let\autoref\cref % set \autoref as an alias for \cref



\usepackage{pifont}



==> tables/tab_eval_breakdown.tex <==


\begin{figure}[h]
\centering
\begin{subfigure}{0.98\linewidth}
      \centering
      % include first image
      \includegraphics[width=\linewidth]{figures/uxcost_stage.jpg}
      \caption{UXCost breakdown figure}
      \label{fig:uxcost_stages}
\end{subfigure}
\hfill
\begin{subfigure}{0.98\linewidth}
\resizebox{0.48\textwidth}{!}{%i
\centering
\begin{tabular}{|c|c|c|} 
\hline
                & 4K PE  & 8K PE   \\ 
\hhline{|===|}
\begin{tabular}[c]{@{}c@{}}Default\\(\alpha,\beta=1)\end{tabular} & 1 & 1  \\ 
\hline
MapScore        & 0.49 & 0.21  \\
SmartDrop       & 0.17 & 0.14  \\
\begin{tabular}[c]{@{}c@{}}Supernet\\Switch\end{tabular} & 0.06  & 0.09   \\
\hline
Total        & 0.72 & 0.44  \\
\hline
\end{tabular}
}
\caption{Area breakdown.}
\label{tab:uxcost-breakdown}
\end{subfigure}
\caption{\textcolor{green}{\costFunction improvement breakdown for each optimization method. The result uses geomean of \vr and \ar.}}
\label{tab:uxcost-breakdown}
\end{figure}
